Designing a Provenance Analysis for SGX Enclaves

Intel SGX enables memory isolation and static integrity verification of code and data stored in user-space memory regions called enclaves. SGX effectively shields the execution of enclaves from the underlying untrusted OS. Attackers cannot tamper nor examine enclaves' content. However, these properties equally challenge defenders as they are precluded from any provenance analysis to infer intrusions inside SGX enclaves. In this work, we propose SgxMonitor, a novel provenance analysis to monitor and identify anomalous executions of enclave code. To this end, we design a technique to extract contextual runtime information from an enclave and propose a novel model to represent enclaves' intrusions. Our experiments show that not only SgxMonitor incurs an overhead comparable to traditional provenance tools, but it also exhibits macro-benchmarks' overheads and slowdowns that marginally affect real use cases deployment. Our evaluation shows SgxMonitor successfully identifies enclave intrusions carried out by the state of the art attacks while reporting no false positives and negatives during normal enclaves executions, thus supporting the use of SgxMonitor in realistic scenarios.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

%% **FLAVIO**: I guess all the following section and introduction should be 
%% removed and made smoothier.

%\sgxmonitor{} mitigates control-flow manipulations of SGX enclaves.
%Here, we describe the current code-reuse attacks against SGX
%(Section~\ref{ssec:sota-attacks}), analyze their causes 
%(Section~\ref{ssec:limits}), and formalize our threat model 
%(Section~\ref{sec:threat-model}).

%\subsection{Current SGX Code-Reuse Attacks}
%\label{ssec:sota-attacks}
%
%Performing code-reuse attacks against enclaves is challenging 
%due to the SGX isolation.
%The following works propose methods to craft code-reuse payloads for
%enclaves.
%
%\paragraph{Dark-ROP}
%Lee et. al present Dark-ROP~\cite{lee2017hacking}, a technique to locate 
%gadgets in an enclave.
%In their scenario, the attacker probes
%a victim enclave until triggering an \texttt{AEX}.
%From the exception risen, the host can gain information about the location and 
%the nature of the gadgets.
%Once enough gadgets are collected, the adversary can finally craft a payload 
%and bypass the enclave protections.
%The success of this technique exploits the fact that neither the enclave 
%nor an external observer (\eg the microcode) can backtrack the cause of a 
%crash.
%In practice, the SGX isolation does not allow inspection either for 
%\emph{good} analysis or by adversaries.
%
%\paragraph{Guard's Dilemma}
%Biondo et. al propose a new approach, called \emph{Guard's Dilemma}, that does 
%not require probing the enclave~\cite{biondo2018guard}.
%The authors abuse two critical Intel SGX SDK procedures to control the CPU 
%registers.
%The first one is \texttt{asm\_oret}, that restores the CPU registers after an  
%OCALL.
%The second one is \texttt{continue\_execution}, that is used in the exception
%handling.
%The authors use the latter to perform a stack pivoting (\ie control the 
%\texttt{rsp} register).
%\emph{Dilemma} works because the enclave has no mechanism to validate
%the integrity of the input of these two functions.

%\subsection{Limit of SGX and \sgxmonitor{} Philosophy}
%\label{ssec:limits}

%\todo{discuss about CFG bypassable but we have this cat and mouse game! since 
%I 
%assume malicious execution can happens, we move to runtime RA to monitor and 
%get prof the execution. But we can't actually, we need a model and a design.
%Our challenge sono automatico model e noi usiamo symexe + static to model 
%enclave becacuse the enclave programs are small (a predictable behavior).}

%% **MOVED INTO INTRODUCTION**
\textcolor{red}{
The SGX isolation pushed researchers to find new techniques for bending the 
enclave 
execution~\cite{251582,biondo2018guard,lee2017hacking,tale-two-worlds,snakegx,alder2020faulty}.
Historically, possible solutions for these attacks combine program
analysis (to learn the \emph{correct} program behavior) and 
anomaly detection techniques (to spot deviation from the \emph{correct} 
behavior)~\cite{wagner2000intrusion,feng2003anomaly,mutz2006anomalous,924295}.
However, deploying these strategies over general purpose software (such as 
video games or database management systems) introduces imprecision issues that 
lead to an high rate of false positives and negatives.}
\textcolor{red}{
These imprecision is inherited from program analysis, that struggle to scale 
over large portion of code~\cite{hind1999interprocedural,lattner2007making}.
On the contrary, we argue that SGX enclaves are designed for containing a 
relatively short but sensitive pieces of code~\cite{intel2}, and thus suitable 
to be automatically modelled through a combination of symbolic execution and 
static analysis while producing very low false positives and negatives.}


%% **MOVED INTO MODEL**
\textcolor{red}{
On top of the classic anomaly detection limitations, the SGX isolation 
introduces extra challenges, \ie it avoids legit users to validate the 
runtime integrity of an enclave, thus recognizing the presence of attacks.}
To understand the underlying reason of this limit, we analyze the SGX 
enclave life-cycle, which is depicted as a Finite-State-Machine in 
Figure~\ref{fig:fmi-standard}.\footnote{This model is a simplified version 
of~\cite{costan2016intel}.}
We assume the enclave has been loaded correctly and the host 
interacts with it by means of the opcodes described in 
Section~\ref{sec:background}.
The model allows the enclave state to assume only two values: 
\emph{non-in-use} and \emph{in-use}.
In particular, an enclave transits to \emph{in-use} state when an 
\texttt{EENTER} or \texttt{ERESUME} is issued.
Then, the state returns to \emph{non-in-use} when an \texttt{EEXIT} or  
\texttt{AEX} happens.
This simple model is already implemented in the microcode: the same thread 
cannot enter (\ie \texttt{EENTER}) in an enclave which is 
already in \emph{in-use} state; it cannot exit (\ie \texttt{EEXIT}) when the 
enclave is in \emph{non-in-use}.

Intuitively, this model provides limited information about the enclave health.
\stbold{In case of Dark-ROP or Dilemma,} 
\newtxt{In case of new enclave 
attacks}~\cite{lee2017hacking,biondo2018guard,snakegx}, we are not able to 
backtrace the enclave execution, and finally, distinguish whether an enclave 
has been executed properly or not.
To mitigate these issues, one might implement stronger defenses inside 
the enclave. However, the defenses are prone of errors as 
well~\cite{biondo2018guard,lee2017hacking,tale-two-worlds,251582},
which leads to a complex arms-race.
With \sgxmonitor{}, we embrace an orthogonal approach that assumes the 
possibility of malicious executions. Our proposal is to continuously 
monitor the enclave and provides proofs of correct execution.
Ideally, we would like to have only \emph{benign} enclave inspections, without
leaving rooms for threats.
On the other hand, providing a secure inspection technique, which is able to 
preserve the SGX privacy properties, is anything but an easy task.
\sgxmonitor{} extends the model in Figure~\ref{fig:fmi-standard} to verify 
correct
enclaves runtime behavior, thus embracing the SGX security 
guarantees.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{img/fmi-standard}
	\caption{Standard Finite-State-Machine representation of SGX 
	Enclave~\cite{costan2016intel}.}
	\label{fig:fmi-standard}
\end{figure}

%\subsection{SGX Remote Attestation}
%\label{ssec:sgx-ra}
%\todo{thinking whether to remove this section.}
%%\todo{I should add few lines for sgx remote attestation, or maybe not?}
%
%SGX Remote Attestation (SGX RA) is a protocol that allows an entity to 
%validate 
%the integrity of a remote enclave (\ie an enclave loaded on a remote machine).
%The outcome of this protocol is a fresh measurement (\ie a cryptography hash 
%value) that represents the pages of the loaded enclave.
%This mechanisms, combined with the hardware isolation, allows one to exchange 
%a 
%secret with a remote enclave and verifies the remote enclave 
%identity~\todo{cite}.
%For instance, Signal uses an enclave to perform contact discovering without
%reveling private contact information into the cloud.
%
%SGX RA is called static because it can only represent static 
%properties (\ie the software loaded), while it cannot represent the integrity
%of runtime structures, that might be manipulated by code-reuse attacks.
%In the recent years, researchers and practitioners proposed runtime RA 
%schemes  
%that cope with static RA limitations~\todo{cite}.
%However, current techniques are not suitable for the SGX realm for many 
%reasons:
%\begin{enumerate*}[label=(\roman*)]
%	\item they do not model TEE internal state;
%	\item they require an independent TEE (while SGX assumes the entire 
%	host is compromised);
%	\item it is not possible to inspect an enclave runtime state.
%\end{enumerate*}

